Cerberus: Multi-Agent Reasoning and Coverage-Guided Exploration for Static Detection of Runtime Errors

In several software development scenarios, it is desirable to detect runtime errors and exceptions in code snippets without actual execution. A typical example is to detect runtime exceptions in online code snippets before integrating them into a codebase. In this paper, we propose Cerberus, a novel predictive, execution-free coverage-guided testing framework. Cerberus uses LLMs to generate the inputs that trigger runtime errors and to perform code coverage prediction and error detection without code execution. With a two-phase feedback loop, Cerberus first aims to both increasing code coverage and detecting runtime errors, then shifts to focus only detecting runtime errors when the coverage reaches 100% or its maximum, enabling it to perform better than prompting the LLMs for both purposes. Our empirical evaluation demonstrates that Cerberus performs better than conventional and learning-based testing frameworks for (in)complete code snippets by generating high-coverage test cases more efficiently, leading to the discovery of more runtime errors.

==> rq4-r2.tex <==
%\section{Fuzzing on an S/O code - A Case Study}
%\label{sec:rq5}



%(*@{\color{blue}Code Snippet from StackOverflow@*)

\begin{figure}[t]
  \centering
	\lstset{
		numbers=left,
		numberstyle= \tiny,
		keywordstyle= \color{blue!70},
		commentstyle= \color{red!50!green!50!blue!50},
		frame=shadowbox,
		rulesepcolor= \color{red!20!green!20!blue!20} ,
		xleftmargin=1.5em,xrightmargin=0em, aboveskip=1em,
		framexleftmargin=1.5em,
                numbersep= 5pt,
		language=Java,
    basicstyle=\scriptsize\ttfamily,
    numberstyle=\scriptsize\ttfamily,
    emphstyle=\bfseries,
                moredelim=**[is][\color{red}]{@}{@},
		escapeinside= {(*@}{@*)}
	}
%\begin{minipage}{\textwidth}        
\begin{lstlisting}[caption = ]
from pytube import YouTube
link = input("Enter the link of YouTube video you want to download:  ")
yt = YouTube(link)
print("Title: ",yt.title)
print("Number of views: ",yt.views)
print("Length of video: ",yt.length)
print("Rating of video: ",yt.rating)
ys = yt.streams.get_highest_resolution()
print("Downloading...")
ys.download()
print("Download completed!!")
\end{lstlisting}
%\end{minipage}
\vspace{-15pt}
\caption{Runtime Error in a Stack Overflow Code Snippet}
\label{fig:rq5-stackoverflow-code}
\end{figure}

%Real-world code frequently encounters various issues that lead to errors and bugs, affecting its functionality and reliability. Common problems include missing imports, where the code references functions or classes that have not been imported, resulting in NameError during execution.Additionally, outdated or poorly maintained libraries may contain known bugs or lack support for specific features, and updating these libraries to the latest versions can often resolve these issues. Another prevalent issue is missing variable dependencies, where variables used within functions are not defined in the proper scope, leading to UnboundLocalError. The objective of this case study is to evaluate whether Cerberus can maintain the standards set by previous research questions when applied to real-world code.

\subsection{Case Study}

Let us explain {\tool}'s use in a case study. Fig~\ref{fig:rq5-stackoverflow-code} displays the code
snippet in the S/O post
\#76654129~\cite{stackoverflow-casestudy}. This Python script uses the
\code{pytube} library to download a YouTube video by prompting the
user for the URL. It retrieves the YouTube video to display
metadata.

This Stack Overflow code snippet contains two notable runtime errors. The first is a \code{ModuleNotFoundError}, triggered by the call to \code{YouTube(.)} at line 3 when an invalid URL is provided as input. A fuzzer's objective in this case is to generate an input YouTube link that causes this runtime error. The second issue lies within the \code{pytube} library itself. A bug in the internal function \code{get\_throttling\_function\_} \code{name} causes a \code{RegexMatchError} exception~\cite{youtube-error}, which occurs immediately after the Python interpreter executes the import statement at line 1, \code{from pytube import YouTube}. Consequently, any fuzzer that relies on actual execution will fail to progress beyond the first line and will be unable to detect the \code{ModuleNotFoundError} exception, regardless of the input. In essence, the presence of the first line renders the code snippet non-executable, leading other fuzzers to fail.

%is a runtime error in the \code{pytube}~library. It was reported that
%the internal function \code{get\_throttling\_function\_name} could not
%find a match for {\em certain input youtube links}, thus, throwing an
%\code{RegexMatchError} exception~\cite{youtube-error}. The goal of a
%fuzzer is to produce such an input youtube link to trigger that
%runtime error.
%
%However, there is another runtime error in the \code{pytube} library
%that throws a \code{ModuleNotFoundError} when the first line (i.e.,
%the import statement) was executed. Therefore, any other fuzzer that
%requires actual execution will not be able to get pass the first line,
%i.e., cannot detect the \code{RegexMatchError} exception. In other
%words, the presence of the first line makes the code snippet {\em
%  non-executable}.
 
When this S/O snippet was fuzzed with {\tool}, it 
produces two Youtube URL inputs:

1) \code{https://www.youtube.com/watch?v=INVALIDLINK} to bypass the
import statement and to detect the \code{ModuleNotFoundError} exception at
line 3: \code{YouTube(link)}.

2) ``Test1234'' to trigger \code{RegexMatchError}  and to
point to the \code{import} statement as an error.

This shows that {\tool} can handle code snippets. Also, with its pre-trained knowledge, LLM can reason on the API \code{YouTube(.)} despite the error at line 1. Existing fuzzers that rely on actual execution are ineffective in this case.


%it generates invalid YouTube URLs (refer to
%Fig.~\ref{fig:rq5-invalidURL}) that would have thrown a
%RegexMatchError if the import statement were non-buggy. Additionally,
%{\tool} is not only able to generate valid YouTube URLs (refer to
%Fig.~\ref{fig:rq5-validURL}) that would pass the code snippet without
%any errors, but also predict the ModuleNotFoundError, along with
%reasoning that the import statement could be the cause for this error
%(refer to Fig.~\ref{fig:rq5-importerror}). This demonstrates {\tool}'s
%ability to handle real-world code issues effectively.


%Consider the code snippet from a StackOverflow post ({\color{blue} add url to post}) illustrated in Fig. ~\ref{fig:rq5-stackoverflow-code}. This Python script uses the pytube library to download a YouTube video by prompting the user for the video URL. It creates a YouTube object to access and display metadata about the video, such as its title, number of views, length, and rating. The script selects the stream with the highest resolution and proceeds to download the video, indicating the start and completion of the download process.

%Notably, the pytube library has a bug ({\color{blue}refer to the github url link added in reference}). which causes a ModuleNotFoundError when the code is executed.

%Irrespective of whether the test case input (Youtube link) is valid or invalid, the code snippet in Fig. ~\ref{fig:rq5-stackoverflow-code} throws a ModuleNotFoundError everytime it is executed, thus rendering the remainder of the code untestable. 



%============ Tien removed this figure =====
%\begin{figure}[t]
%  \centering
%	\lstset{
%		numbers=left,
%		numberstyle= \tiny,
%		keywordstyle= \color{blue!70},
%		commentstyle= \color{red!50!green!50!blue!50},
%		frame=shadowbox,
%		rulesepcolor= \color{red!20!green!20!blue!20} ,
%		xleftmargin=1.5em,xrightmargin=0em, aboveskip=1em,
%		framexleftmargin=1.5em,
%                numbersep= 5pt,
%		language=Java,
%    basicstyle=\scriptsize\ttfamily,
%    numberstyle=\scriptsize\ttfamily,
%    emphstyle=\bfseries,
%                moredelim=**[is][\color{red}]{@}{@},
%		escapeinside= {(*@}{@*)}
%	}
%\begin{minipage}{.45\textwidth}        
%\begin{lstlisting}[caption = ]
%(*@{\color{orange}Test Case generated by LLM A} @*)
%(*@{\color{blue}INPUT : https://www.youtube.com/watch?v=INVALIDLINK } @*)
%(*@{\color{orange}{\model}'s Prediction} @*)
%PLAN:
%1. Import statement: The statement from pytube import YouTube is executed.
%2. User Input: The statement link = input(...) is executed to get the link from the user.
%3. YouTube object creation: The statement yt = YouTube(link) is executed but fails due to an invalid link.
%4. Showing details: Since the creation of the YouTube object failed, none of the print statements for showing details are executed.
%5. Getting the highest resolution: The statement ys = yt.streams.get_highest_resolution() is not executed because the yt object was not successfully created.
%6. Starting download: The print statement "Downloading..." and ys.download() are not executed because the program failed before reaching this point.
%7. Download completed: The print statement "Download completed!!" is not executed due to the failure in creating the yt object.
%
%FINAL PREDICTED CODE COVERAGE:
%> from pytube import YouTube
%> link = input("Enter the link of YouTube video you want to download:  ")
%! yt = YouTube(link)
%! print("Title: ",yt.title)
%! print("Number of views: ",yt.views)
%! print("Length of video: ",yt.length)
%! print("Rating of video: ",yt.rating)
%! ys = yt.streams.get_highest_resolution()
%! print("Downloading...")
%! ys.download()
%! print("Download completed!!")
%
%EXPECTED OUTPUT - An error related to the failure in creating a YouTube object with an invalid link, possibly a pytube.exceptions.RegexMatchError
%(*@{\color{orange}Result on Execution} @*)
%from pytube import YouTube\nModuleNotFoundError: No module named 'pytube'
%\end{lstlisting}
%\end{minipage}
%\vspace{-6pt}
%\caption{Fuzzing with Invalid URL input (Generated by LLM A)}
%\label{fig:rq5-invalidURL}
%\end{figure}


%============== Tien removed this ===============
%\begin{figure}[t]
%  \centering
%	\lstset{
%		numbers=left,
%		numberstyle= \tiny,
%		keywordstyle= \color{blue!70},
%		commentstyle= \color{red!50!green!50!blue!50},
%		frame=shadowbox,
%		rulesepcolor= \color{red!20!green!20!blue!20} ,
%		xleftmargin=1.5em,xrightmargin=0em, aboveskip=1em,
%		framexleftmargin=1.5em,
%                numbersep= 5pt,
%		language=Java,
%    basicstyle=\scriptsize\ttfamily,
%    numberstyle=\scriptsize\ttfamily,
%    emphstyle=\bfseries,
%                moredelim=**[is][\color{red}]{@}{@},
%		escapeinside= {(*@}{@*)}
%	}
%\begin{minipage}{.45\textwidth}        
%\begin{lstlisting}[caption = ]
%(*@{\color{orange}Test Case generated by LLM A} @*)
%(*@{\color{blue}INPUT : https://www.youtube.com/watch?v=dQw4w9WgXcQ } @*)
%(*@{\color{orange}{\model}'s Prediction} @*)
%PLAN for step by step execution:
%1. Import statement: The statement from pytube import YouTube is executed.
%2. User Input: The statement link = input("Enter the link of YouTube video you want to download:  ") is executed.
%3. YouTube object creation: yt = YouTube(link) is executed.
%4. Showing details: Statements to print video details (title, views, length, rating) are executed.
%5. Getting the highest resolution: ys = yt.streams.get_highest_resolution() is executed.
%6. Starting download: The print statement "Downloading..." is executed.
%7. Video download: ys.download() is executed.
%8. Download completed: The print statement "Download completed!!" is executed.
%
%Final code coverage of the Python program based on its test case:
%> from pytube import YouTube
%> link = input("Enter the link of YouTube video you want to download:  ")
%> yt = YouTube(link)
%> print("Title: ",yt.title)
%> print("Number of views: ",yt.views)
%> print("Length of video: ",yt.length)
%> print("Rating of video: ",yt.rating)
%> ys = yt.streams.get_highest_resolution()
%> print("Downloading...")
%> ys.download()
%> print("Download completed!!")
%
%EXPECTED OUTPUT - Since the test case is a valid YouTube link, there should be no error or exception, and the video should be downloaded successfully.
%(*@{\color{orange}Result on Execution} @*)
%from pytube import YouTube\nModuleNotFoundError: No module named 'pytube'
%\end{lstlisting}
%\end{minipage}
%\vspace{-6pt}
%\caption{Fuzzing with Valid URL input (Generated by LLM A)}
%\label{fig:rq5-validURL}
%\end{figure}

%=================== Tien removed this too ============
%\begin{figure}[t]
%  \centering
%	\lstset{
%		numbers=left,
%		numberstyle= \tiny,
%		keywordstyle= \color{blue!70},
%		commentstyle= \color{red!50!green!50!blue!50},
%		frame=shadowbox,
%		rulesepcolor= \color{red!20!green!20!blue!20} ,
%		xleftmargin=1.5em,xrightmargin=0em, aboveskip=1em,
%		framexleftmargin=1.5em,
%                numbersep= 5pt,
%		language=Java,
%    basicstyle=\scriptsize\ttfamily,
%    numberstyle=\scriptsize\ttfamily,
%    emphstyle=\bfseries,
%                moredelim=**[is][\color{red}]{@}{@},
%		escapeinside= {(*@}{@*)}
%	}
%\begin{minipage}{.45\textwidth}        
%\begin{lstlisting}[caption = ]
%(*@{\color{orange}Test Case generated by LLM A} @*)
%(*@{\color{blue}INPUT : Test1234 } @*)
%(*@{\color{orange}{\model}'s Prediction} @*)
%PLAN:
%1. Import statement: The statement from pytube import YouTube is not executed.
%2. User Input: Statements link = input("Enter the link of YouTube video you want to download:  ") is not executed.
%3. YouTube object creation: The statement yt = YouTube(link) is executed but will fail due to ModuleNotFoundError.
%4. Showing details: Since the creation of YouTube object failed, none of the print statements regarding video details will be executed.
%5. Getting the highest resolution: The statement ys = yt.streams.get_highest_resolution() will not be executed due to prior error.
%6. Starting download: The print statement for starting download and ys.download() will not be executed due to prior error.
%7. Completion message: The final print statement indicating download completion will not be executed due to prior error.
%
%PREDICTED CODE COVERAGE:
%! from pytube import YouTube
%! link = input("Enter the link of YouTube video you want to download:  ")
%! yt = YouTube(link)
%! print("Title: ",yt.title)
%! print("Number of views: ",yt.views)
%! print("Length of video: ",yt.length)
%! print("Rating of video: ",yt.rating)
%! ys = yt.streams.get_highest_resolution()
%! print("Downloading...")
%! ys.download()
%! print("Download completed!!")
%
%EXPECTED OUTPUT - ModuleNotFoundError
%(*@{\color{orange}Result on Execution} @*)
%from pytube import YouTube\nModuleNotFoundError: No module named 'pytube'
%\end{lstlisting}
%\end{minipage}
%\vspace{-6pt}
%\caption{{\tool} Detecting ModuleNotFoundError}
%\label{fig:rq5-importerror}
%\end{figure}

